Incremental Few-Shot Object Detection for Robotics

Incremental few-shot learning is highly expected for practical robotics applications. On one hand, robot is desired to learn new tasks quickly and flexibly using only few annotated training samples; on the other hand, such new additional tasks should be learned in a continuous and incremental manner without forgetting the previous learned knowledge dramatically. In this work, we propose a novel Class-Incremental Few-Shot Object Detection (CI-FSOD) framework that enables deep object detection network to perform effective continual learning from just few-shot samples without re-accessing the previous training data. We achieve this by equipping the widely-used Faster-RCNN detector with three elegant components. Firstly, to best preserve performance on the pre-trained base classes, we propose a novel Dual-Embedding-Space (DES) architecture which decouples the representation learning of base and novel categories into different spaces. Secondly, to mitigate the catastrophic forgetting on the accumulated novel classes, we propose a Sequential Model Fusion (SMF) method, which is able to achieve long-term memory without additional storage cost. Thirdly, to promote inter-task class separation in feature space, we propose a novel regularization technique that extends the classification boundary further away from the previous classes to avoid misclassification. Overall, our framework is simple yet effective and outperforms the previous SOTA with a significant margin of 2.4 points in AP performance.

==> table.tex <==
\begin{table}
\small
\setlength{\tabcolsep}{0.7mm}{

 \begin{tabular}{*{22}{c}}

    \toprule
        & \multirow{1.5}{*}{\thead{Shots}} 
      

        & \multirow{1.5}{*}{\thead{Methods}} 
        & 
        &
      
       
            &   \multicolumn{3}{c}{\thead{Novel split 1}} 
            &
            &
            &
                & \multicolumn{3}{c}{\thead{Novel split 2}}
                &
                &
                &
                & \multicolumn{3}{c}{\thead{Novel split 3}}\\
    \cmidrule(l){4-9}   \cmidrule(l){10-15} \cmidrule(l){16-21}
    &    &   &     & bird    & bus   & cow   &sofa &mbike & & aero    & bottle    & cow &horse  &sofa&  &sheep& boat    & cat &sofa   & mbike    \\ 
    \midrule
 &  & YOLO-LS  &   & 00.0    & 00.0    & 00.0 &00.0 &00.0 &  & 00.0    & 00.0    & 00.0 &00.0 &00.0& & 00.0    & 00.0   & 00.0  &00.0   &00.0\\
   &  & Meta-RCNN &   & 00.0    & 00.0    & 00.0 &00.0 &00.0 &  & 00.0    & 00.0    & 00.0 &00.0 &00.0& & 00.0    & 00.0   & 00.0  &00.0   &00.0\\
   & 3 & FRCN-joint &   & 00.0    & 00.0    & 00.0 &00.0 &00.0 &  & 00.0    & 00.0    & 00.0 &00.0 &00.0& & 00.0    & 00.0   & 00.0  &00.0   &00.0\\
   &  & FRCN-ft  &   & 00.0    & 00.0    & 00.0 &00.0 &00.0 &  & 00.0    & 00.0    & 00.0 &00.0 &00.0& & 00.0    & 00.0   & 00.0  &00.0   &00.0\\
    &  & FRCN-ft+DCR  &   & 00.0    & 00.0    & 00.0 &00.0 &00.0 &  & 00.0    & 00.0    & 00.0 &00.0 &00.0& & 00.0    & 00.0   & 00.0  &00.0   &00.0\\
    &  & FRCN-ft+LSCN  &   & 00.0    & 00.0    & 00.0 &00.0 &00.0 &  & 00.0    & 00.0    & 00.0 &00.0 &00.0& & 00.0    & 00.0   & 00.0  &00.0   &00.0\\
    \midrule
 &  & YOLO-LS  &   & 00.0    & 00.0    & 00.0 &00.0 &00.0 &  & 00.0    & 00.0    & 00.0 &00.0 &00.0& & 00.0    & 00.0   & 00.0  &00.0   &00.0\\
   &  & Meta-RCNN  &   & 00.0    & 00.0    & 00.0 &00.0 &00.0 &  & 00.0    & 00.0    & 00.0 &00.0 &00.0& & 00.0    & 00.0   & 00.0  &00.0   &00.0\\
   & 10 & FRCN-joint &   & 00.0    & 00.0    & 00.0 &00.0 &00.0 &  & 00.0    & 00.0    & 00.0 &00.0 &00.0& & 00.0    & 00.0   & 00.0  &00.0   &00.0\\
   &  & FRCN-ft  &   & 00.0    & 00.0    & 00.0 &00.0 &00.0 &  & 00.0    & 00.0    & 00.0 &00.0 &00.0& & 00.0    & 00.0   & 00.0  &00.0   &00.0\\
    &  & FRCN-ft+DCR  &   & 00.0    & 00.0    & 00.0 &00.0 &00.0 &  & 00.0    & 00.0    & 00.0 &00.0 &00.0& & 00.0    & 00.0   & 00.0  &00.0   &00.0\\
    &  & FRCN-ft+LSCN &   & 00.0    & 00.0    & 00.0 &00.0 &00.0 &  & 00.0    & 00.0    & 00.0 &00.0 &00.0& & 00.0    & 00.0   & 00.0  &00.0   &00.0\\
    \bottomrule
    
    
    
    
    \end{tabular}}
    
    
    
\end{table}


\begin{table}

\setlength{\tabcolsep}{1mm}{

 \begin{tabular}{*{22}{c}}

    \toprule
        & \multirow{1}{*}{\thead{Shots}}  & \multirow{1}{*}{\thead{Methods}} 

    &        & AP    & AP50   & AP75   &APS &APM &  APL   & & &AR1    & AR10 &AR100  &ARS&  ARM& ARL   \\ 
    \midrule
 &  & YOLO-LS  &   & 00.0    & 00.0    & 00.0 &00.0 &00.0   & 00.0 &   && 00.0    & 00.0 &00.0 &00.0 & 00.0    & 00.0   \\
   &  & Meta-RCNN &   & 00.0    & 00.0    & 00.0 &00.0 &00.0   & 00.0 & &  & 00.0    & 00.0 &00.0 &00.0 & 00.0    & 00.0   \\
   & 10 & FRCN-joint &   & 00.0    & 00.0    & 00.0 &00.0 &00.0   & 00.0 &  & & 00.0    & 00.0 &00.0 &00.0&  00.0    & 00.0   \\
   &  & FRCN-ft  &   & 00.0    & 00.0    & 00.0 &00.0 &00.0   & 00.0 &  & & 00.0    & 00.0 &00.0 &00.0&  00.0    & 00.0   \\
    &  & FRCN-ft+DCR  &   & 00.0    & 00.0    & 00.0 &00.0 &00.0   & 00.0 &  & & 00.0    & 00.0 &00.0 &00.0&  00.0    & 00.0   \\
    &  & FRCN-ft+LSCN  &   & 00.0    & 00.0    & 00.0 &00.0 &00.0   & 00.0 & &  & 00.0    & 00.0 &00.0 &00.0&  00.0    & 00.0   \\
    \midrule
 &  & YOLO-LS  &   & 00.0    & 00.0    & 00.0 &00.0 &00.0   & 00.0 &   && 00.0    & 00.0 &00.0 &00.0 & 00.0    & 00.0   \\
   &  & Meta-RCNN &   & 00.0    & 00.0    & 00.0 &00.0 &00.0   & 00.0 &   && 00.0    & 00.0 &00.0 &00.0 & 00.0    & 00.0   \\
   & 30 & FRCN-joint &   & 00.0    & 00.0    & 00.0 &00.0 &00.0   & 00.0 &   && 00.0    & 00.0 &00.0 &00.0 & 00.0    & 00.0   \\
   &  & FRCN-ft  &   & 00.0    & 00.0    & 00.0 &00.0 &00.0   & 00.0 &   && 00.0    & 00.0 &00.0 &00.0 & 00.0    & 00.0   \\
    &  & FRCN-ft+DCR &   & 00.0    & 00.0    & 00.0 &00.0 &00.0   & 00.0 &   && 00.0    & 00.0 &00.0 &00.0 & 00.0    & 00.0   \\
    &  & FRCN-ft+LSCN &   & 00.0    & 00.0    & 00.0 &00.0 &00.0   & 00.0 &   && 00.0    & 00.0 &00.0 &00.0 & 00.0    & 00.0   \\
    \bottomrule
    
    
    
    
    \end{tabular}}
    
    
    
\end{table}
